TOVAC: Tele-operated Vehicle Admission Control and Routing

Tele-operated Driving (ToD) is a challenging use case for mobile network operators. Video captured by the built-in vehicle cameras must be streamed meeting a latency requirement of 5 ms with a 99.999% reliability. Although 5G offers high bandwidth, ultra-low latencies and high reliability; ToD service requirements are violated due to bad channel conditions. Ignoring the channel state may lead to over-estimate the number of ToD vehicles that can meet the service requirements, hence comprising the vehicle security. To fill this gap, in this letter we propose TOVAC, an algorithm that guarantees ToD service requirements by taking adequate admission control and routing decisions. This is achieved by using a channel-based capacity graph that determines the maximum number of vehicles that can be tele-operated in any road section. We evaluate TOVAC considering cellular deployments from Turin and show that, unlike a state of the art solution, TOVAC guarantees the ToD service requirements.

==> carlos-illustration.tex <==

%%%%%%%%%%%%%%%%%
%% Second figure. Depicting the violation of the Packect Delay Budget
%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        % Axis
        \draw[->] (-.3,-.2) -- (8,-.2)
            node[anchor=west] {$t$};
        \draw[->] (-.3,3) -- (8,3)
            node[anchor=west] {$t$};
        \draw[->] (-.3,-.2) -- (-.3,5)
            node[anchor=south,
            rotate=90] {freq.};


        %%%%%%%%%%%%%%%%
        %%% VEHICLE 4 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=green!30, draw opacity=0.5] (0.75,0.75) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=green!30, draw opacity=0.5] (0.75,1.75) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (1.4,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_3}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 3 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=blue!30, draw opacity=0.4] (0.5,0.5) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=blue!30, draw opacity=0.4] (0.5,1.5) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (1.4,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_3}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 2 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=red!30, draw opacity=0.3] (0.25,0.25) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=red!30, draw opacity=0.3] (0.25,1.25) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (0.125,0.125) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_2}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 1 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=gray!30, opacity=1] (0,0) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=gray!30, opacity=1] (0,1) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (-.1,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_1}$};



        %%%%%%%%%%%%%%%%
        %%% VEHICLE 4 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=green!30, draw opacity=0.5] (3.75,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=green!30, draw opacity=0.5] (3.75,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (1.4,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_3}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 3 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=blue!30, draw opacity=0.4] (2.5,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=blue!30, draw opacity=0.4] (2.5,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (1.4,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_3}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 2 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=red!30, draw opacity=0.3] (1.25,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=red!30, draw opacity=0.3] (1.25,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (0.125,0.125) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_2}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 1 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=gray!30, opacity=1] (0,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=gray!30, opacity=1] (0,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (-.1,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_1}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 2 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=red!30, draw opacity=0.3] (6.25,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=red!30, draw opacity=0.3] (6.25,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (0.125,0.125) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_2}$};

        %%%%%%%%%%%%%%%%
        %%% VEHICLE 1 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=gray!30, opacity=1] (5,3) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{1}};
        \draw[black,fill=gray!30, opacity=1] (5,4) rectangle ++(1,1)
            node[anchor=north east] {PRB\textsubscript{2}};
        % UDP packet
        %\draw[black,dashed] (-.1,-.1) rectangle ++(1.2,2.2)
        %    node[anchor=south east]  {UDP$_{\nu_1}$};

        % Window D
        \draw[black,dashed] (-.1,2.9) rectangle ++(4.95,2.2)
            node[anchor=south east] {};

       
        % PDB
        \draw[<->] (-.125,6) -- (3.6125,6)
            node[pos=0.5,anchor=south]
            {$D=5$ ms};
        \draw[dotted] (3.6125,0) -- (3.6125,6);

        \draw[<->] (3.6125,6) -- (7.35,6)
            node[pos=0.5,anchor=south]
            {$D=5$ ms};
        \draw[dotted] (7.35,0) -- (7.35,6);

        % Tx and Tw
        \draw[<->] (-.125,-.5) -- (3.6125,-.5)
            node[pos=0.5,anchor=north]
            {$T_w$};
        \draw[<->] (3.6125,-.5) -- (4.75,-.5)
            node[pos=0.5,anchor=north]
            {$T_x$};

    \end{tikzpicture}

    
    \caption{Fig. 2 shows the problem that arises if the admission control that we are proposing is not used. Consider the situation where all the vehicles start to transmit at the same time. In this situation, the gNB scheduler will distribute the available PRBs, in a time window of D~ms, between all of the vehicles. However, the number of vehicles wanting to transmit data is greater than the number of vehicles that can transmit data in that time of window. Consequently, the gNB scheduler delays the transmission of some of the vehicles which, in turn, it will delay the transmission of all the vehicles of the fleet.
    }
    \label{fig:packet-generation}
\end{figure}


==> fig/graph.tex <==
%% \usetikzlibrary{calc}
%% \def\hor{.8}  % Horizontal node separation
%% \def\ver{.5} % Vertical node separation
\begin{scope}
    %%%%%%%%%%%%%%%%%%%%
    %% STARTING NODES %%
    %%%%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (start2) {};
    \node[anchor=east] at (start2.west) {$s_2$};
    %
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (start1)
        at ($(start2)+(0,\ver)$) {};
    \node[anchor=east] at (start1.west) {$s_1$};
    %
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (start3)
        at ($(start2)-(0,\ver)$) {};
    \node[anchor=east] at (start3.west) {$s_3$};

    %%%%%%%%%%%%%%%%%%
    %% FIRST COLUMN %%
    %%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col1Mid) at
        ($(start2)+(\hor,0)$) {};
    %
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col1Bottom)
        at ($(start3)+(\hor,0)$) {};


    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    %% JOINS TO FIRST COLUMN %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw (start1) -- (col1Mid);
    \draw (start2) -- (col1Mid);
    \draw (start3) -- (col1Bottom);


    %%%%%%%%%%%%%%%%%%%
    %% SECOND COLUMN %%
    %%%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col2Mid) at
        ($(col1Mid)+(\hor,0)$) {};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %% JOINS TO SECOND COLUMN %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw (col1Mid) -- (col2Mid);
    \draw (col1Bottom) -- (col2Mid);


    %%%%%%%%%%%%%%%%%%
    %% THIRD COLUMN %%
    %%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col3Top) at
        ($(col2Mid)+(\hor,\ver)$) {};
    \node[anchor=west] at (col3Top.east) {$d_1$};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    %% JOINS TO THIRD COLUMN %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw (col2Mid) -- (col3Top);

    %%%%%%%%%%%%%%%%%%%
    %% FOURTH COLUMN %%
    %%%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col4Mid) at
        ($(col3Top)+(\hor,-\ver)$) {};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %% JOINS TO FOURTH COLUMN %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw (col2Mid) -- (col4Mid)
        node[midway,fill=white] {\small $e''$};




    %%%%%%%%%%%%%%%%%%
    %% FIFTH COLUMN %%
    %%%%%%%%%%%%%%%%%%
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col5Mid) at
        ($(col4Mid)+(\hor,0)$) {};
    \node[anchor=west] at (col5Mid.east) {$d_2$};
    \node[circle,draw,fill=black,inner sep=0,
        minimum size=2] (col5Bottom) at
        ($(col4Mid)+(\hor,-\ver)$) {};
    \node[anchor=west] at (col5Bottom.east) {$d_3$};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    %% JOINS TO FIFTH COLUMN %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw (col4Mid) -- (col5Mid);
    \draw (col4Mid) -- (col5Bottom);
\end{scope}


==> first-figure.tex <==

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        % Axis
        \draw[->] (-.3,-.2) -- (8,-.2)
            node[anchor=west] {$t$};
        \draw[->] (-.3,-.2) -- (-.3,5)
            node[anchor=south,
            rotate=90] {freq.};




        %%%%%%%%%%%%%%%%
        %%% VEHICLE 1 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black] (0,0) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black] (0,1) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet
        \draw[black,dashed] (-.1,-.1) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_1}$};



        %%%%%%%%%%%%%%%%
        %%% VEHICLE 2 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=1
        \draw[black,fill=gray!30] (0,3) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black,fill=gray!30] (0,4) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet
        \draw[black,dashed] (-.1,2.9) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_2}$};


        %%%%%%%%%%%%%%%%
        %%% VEHICLE 3 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=gray!50] (1.5,0) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black,fill=gray!50] (1.5,1) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet
        \draw[black,dashed] (1.4,-.1) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_3}$};


        
        %%%%%%%%%%%%%%%%
        %%% VEHICLE 1 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=5
        % PRBs @t=5 ms
        \draw[black] (5,0) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black] (5,1) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet @t=5ms
        \draw[black,dashed] (4.9,-.1) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_1}$};


        %%%%%%%%%%%%%%%%
        %%% VEHICLE 2 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=5
        \draw[black,fill=gray!30] (5,3) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black,fill=gray!30] (5,4) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet
        \draw[black,dashed] (4.9,2.9) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_2}$};


        %%%%%%%%%%%%%%%%
        %%% VEHICLE 3 %%
        %%%%%%%%%%%%%%%%
        % PRBs @t=2
        \draw[black,fill=gray!50] (6.5,0) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{1}};
        \draw[black,fill=gray!50] (6.5,1) rectangle ++(1,1)
            node[anchor=north east]
            {PRB\textsubscript{2}};
        % UDP packet
        \draw[black,dashed] (6.4,-.1) rectangle ++(1.2,2.2)
            node[anchor=south east]  {UDP$_{\nu_3}$};




        % Vehicle arrivals
        \draw[->] (-1,-2) --
            node[pos=0,anchor=north] {$\nu_1$}
            (0,-.7);
        \draw[->] (0,-2) --
            node[pos=0,anchor=north] {$\nu_2$}
            (0,-.7);
        \draw[->] (1,-2) --
            node[pos=0,anchor=north] {$\nu_3$}
            (0,-.7);





        % PRB duration
        \draw[<->] (5,-.5) -- (6,-.5)
            node[pos=0.5,anchor=north]
            {$T_S^\mu$ [sec/sym]};

        % PDB
        \draw[<->] (0,6) -- (4.6,6)
            node[pos=0.5,anchor=south]
            {$D=5$ ms};
        \draw[dotted] (4.6,0) -- (4.6,6);

        % Tx and Tw
        \draw[<->] (0,-.5) -- (1,-.5)
            node[pos=0.5,anchor=north]
            {$T_w$};
        \draw[<->] (1.5,-.5) -- (2.5,-.5)
            node[pos=0.5,anchor=north]
            {$T_x$};


        \path[fill=gray!40,line join=round,line cap=round] (2.8,.2) -- (4.5,.2) -- (4.5, 5)
            -- (1.5, 5) -- (1.5, 3)
            -- (2.8, 3);
        \node at (3,4) {other vehicles};

        
    \end{tikzpicture}

    
    \caption{A \gls{tod}-ed vehicle $\nu$
    sends a single UDP packet during each
    \gls{pdb} window $D$, and all vehicles
    request sending traffic at $t=0$.
    The \gls{tod} slice has
    $\sum_j^J \sigma_j N_{PRB}^{r,j,\mu}=4$
    PRBs in an FDD fashion. Vehicle
    $\nu_3$ arrives at $t=0$, thus, it
    has to wait $T_w$ until the other
    vehicles transmit their UDP packets.
    }
    \label{fig:packet-generation}
\end{figure}


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {\gppsouttrue}  % ps
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {\gppdfouttrue} % pdf
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{\gppdfouttrue} % pdf
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {\gppsouttrue}  % ps
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {\gppdfouttrue} % pdf
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {}              % html
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{\gppsouttrue}  % ps
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {\gppsouttrue}  % ps
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {\gppdfouttrue} % pdf
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {\gppdfouttrue} % pdf

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \csname gnuplot@select@driver@\pgfsysdriver\endcsname
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds,fit}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode

\endinput


==> intro-fig.tex <==
\begin{tikzpicture}

    % Estación base
    \node[draw, circle, minimum size=2cm, thick, fill=gray!30] (base_station) at (0, 0) {};
    \node[draw, rectangle, minimum width=0.5cm, minimum height=0.1cm, thick, fill=white] at (base_station.north) {};

    % Antenas
    \foreach \angle in {90, 210, 330} {
        \draw[thick] (base_station.\angle) -- (\angle:1cm);
        \draw[thick, fill=black] (\angle:1cm) circle (0.1cm);
    }
\end{tikzpicture}



==> old-prbs.tex <==

\subsection{\gls{rb}s per UDP packet}
To understand the number of \gls{rb}s that
are needed to send an UDP packet, we must
now how many bits of information each
\gls{rb} carries. We derive the bits
per \gls{rb} checking first the aggregated
capacity of \gls{gnb} $r$, and then divide the
aggregated capacity by the number of
\gls{rb}s.

First, we obtain the
\gls{ul} capacity of the \gls{gnb} $r$ using
\cite[5.1.1-1]{3gppIMT} formula
\begin{equation}
    B_r = \sum_j^J B_r^j = \sum_j^J \alpha \cdot\nu\cdot Q_m\cdot f\cdot R_{\max}\cdot
    \frac{12\cdot N^{r,j,\mu}_{PRB}}{T_S^{\mu}} (1-OH)
\end{equation}
with $\alpha$ the ratio of \gls{ran}
resources in the \gls{ul}, $\nu$ the
number of layers (antennas used),
$f$ the scaling factor,
$R_{\max}$ the maximum transmission
coding rate,
$N_{PRB}^{r,j,\mu}$ the number of \gls{rb}s
available at the component carrier $j$
in \gls{gnb} $r$ using numerology $\mu$,
$T_S^{\mu}$ the average symbol duration
in a subframe with numerology $\mu$,
and $OH$ is the control overhead in the
\gls{ran} transmission.
Note that $B_r^j$ denotes the capacity in
the \gls{cc} $j$.



Second, we obtain the average bits per
\gls{rb} across \gls{cc}s as
\begin{equation}
    B_{r,PRB}^\mu=\frac{1}{|J|} \sum_j^J 
    \frac{B_r^j\ T_S^\mu}{N_{PRB}^{r,j,\mu}}
\end{equation}
expressed in [bits/PRB] unit units.
Consequently, a UDP packet of
$L=1500\cdot8$~bits will consume
$p(L)=\lceil
\frac{L}{B_{r,PRB}^\mu} \rceil$
[PRB/UDP-packet].


==> t-gnuplot-lua-tikz.tex <==
%%
%%  ConTeXt wrapper for gnuplot-tikz style file
%%
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds,fit]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput


==> wait.tex <==
\begin{tikzpicture}



    \draw[->,thick] (0,0) -- (8.5,0) node[anchor=west] {$t$};
    \draw[->,thick,align=left] (0,0) -- (0,1.6) node[anchor=west] {gNB\\RB};

    % Delay budget limits
    \draw[thick,dashed] (1*0.166666+1,0) -- (1*0.166666+1,1.6);
    \draw[thick,dashed] (6*0.166666+6,0) -- (6*0.166666+6,1.6);
    \draw[<->] (.1+1*0.166666+1,1.6) -- node[midway,fill=white] {$D=5$~ms} (-.1+6*0.166666+6,1.6);

    % Bottom row vehicles
    \foreach \y [count=\x] in {myturkish,myyellow,myviolet,myorange,mygreen,myred}
    {%
        \draw[fill=\y] (.1+\x*0.166666+\x, 0.05) rectangle ++(1,0.3);
        \draw[fill=\y] (.1+\x*0.166666+\x, 0.35) rectangle ++(1,0.3);

        % Gray overhead
        \draw[fill=gray!60] (.1+\x*0.166666+\x, 0.05) rectangle ++(3/14,0.3);
        \draw[fill=gray!60] (.1+\x*0.166666+\x, 0.35) rectangle ++(3/14,0.3);

    }


    % Draw the symbol grid@vehicle1
    \foreach \y in {1,...,14}
    {%
        \draw (.1+1*0.166666+1+\y/14, 0.05) -- (.1+1*0.166666+1+\y/14, 0.65);
    }


    % Outatime tx
    \node[fill=myred,inner sep=1pt] at (.1+6*0.166666+6+3/14+0.5*11/14,0.3) {$\nu_{11}$};


    % Top row vehicles
    \foreach \y [count=\x] in {mypink,mygray,myblue,mypurple,myseagreen}
    {%
        \draw[fill=\y] (.1+\x*0.166666+\x, 0.75) rectangle ++(1,0.3);
        \draw[fill=\y] (.1+\x*0.166666+\x, 1.05) rectangle ++(1,0.3);

        % Gray overhead
        \draw[fill=gray!60] (.1+\x*0.166666+\x, 0.75) rectangle ++(3/14,0.3);
        \draw[fill=gray!60] (.1+\x*0.166666+\x, 1.05) rectangle ++(3/14,0.3);

    }


    % vehicle 6 tx
    \node[fill=myblue,inner sep=1pt] at (.1+3*0.166666+3+3/14+0.5*11/14,1.05) {$\nu_6$};
    \node[align=center] at (.1+6*0.166666+6+3/14+0.5*11/14,1.05) {\gls{pdb}\\violation};


    % Vehicle 6
    \draw[->,thick] (0,-1.2) -- (8.5,-1.2) node[anchor=west] {$t$};
    \draw[fill=myblue] (3/14+.1,-1.15) rectangle ++(11/14,.3);
    \draw[fill=myblue] (3/14+.1,-0.85) rectangle ++(11/14,.3);
    \node[fill=myblue,inner sep=1pt] at (3/14+.1+.5*11/14,-0.85) {$\nu_6$};
    % Waiting and tx times
    \draw[|-|] (1.3,-0.85) -- node[midway,fill=white] {$T_w$} (3*0.166666+3,-0.85);
    \draw[|-|] (.1+3*0.166666+3,-0.85) -- node[midway,fill=white] {$T_x$} (.1+3*0.166666+4,-0.85);
    \draw[->] (.2+3*0.166666+4,-1.2) -- (.2+3*0.166666+4,-0.5) node[anchor=north west] {sent};


    % Vehicle 11
    \draw[->,thick] (0,-2.2) -- (8.5,-2.2) node[anchor=west] {$t$};
    \draw[fill=myred] (3/14+.1,-1.85) rectangle ++(11/14,.3);
    \draw[fill=myred] (3/14+.1,-2.15) rectangle ++(11/14,.3);
    \node[fill=myred,inner sep=1pt] at (3/14+.1+.5*11/14,-1.85) {$\nu_{11}$};
    % Waiting and tx times
    \draw[|-|] (1.3,-1.85) -- node[midway,fill=white] {$T_w$} (6*0.166666+6,-1.85);
    \draw[|-|] (.1+6*0.166666+6,-1.85) -- node[midway,fill=white] {$T_x$} (.1+6*0.166666+7,-1.85);
    \draw[->] (.2+6*0.166666+7,-2.2) -- (.2+6*0.166666+7,-1.5) node[anchor=north west] {sent};

    % alloc tx time of 1ms
    \draw[|-|] (.1+6*0.166666+6,-.3) -- node[midway,anchor=north] {$1$~ms} (.1+6*0.166666+7,-.3);



\end{tikzpicture}

